Characterizing Network Requirements for GPU API Remoting in AI Applications

GPU remoting is a promising technique for supporting AI applications. Networking plays a key role in enabling remoting. However, for efficient remoting, the network requirements in terms of latency and bandwidth are unknown. In this paper, we take a GPU-centric approach to derive the minimum latency and bandwidth requirements for GPU remoting, while ensuring no (or little) performance degradation for AI applications. Our study including theoretical model demonstrates that, with careful remoting design, unmodified AI applications can run on the remoting setup using commodity networking hardware without any overhead or even with better performance, with low network demands.

==> Makefile <==
MAIN ?= gpu
DIFF ?= HEAD^
CODE := $(addsuffix .tex,$(filter-out %.tex,$(wildcard code/*)))
FIGS := $(patsubst %.svg,%.pdf,$(wildcard fig/*.svg))
FIG2 := $(patsubst %.eps,%.pdf,$(wildcard fig/*.eps))
PLOT := $(patsubst %.gp,%.eps,$(wildcard data/*.gp))
PLOT1 := $(patsubst %.gp,%.eps,$(wildcard data/ycsb-overall/*.gp) $(wildcard data/ycsbd-timeline/*.gp) \
	$(wildcard data/ycsbc-lat/*.gp) \
	$(wildcard data/motiv/*.gp) \
	$(wildcard data/app/*.gp) \
	$(wildcard data/datasets/*.gp) \
)

BTEX := --bibtex-args="-min-crossrefs=99"
#BTEX := --bibtex-args=""

all: $(DEPS)
#	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)
#	mv latex.out/$(MAIN).pdf .
	latexmk -pdf -f $(MAIN).tex

data: $(DEPS)

diff: $(DEPS)
	@bin/diff.sh $(DIFF)

help:
	echo "..."


#code/%.tex: code/%
#	pygmentize -P tabsize=4 -P mathescape -f latex $^ > $@

#code/fmt.tex:
#pygmentize -f latex -S default > $@

fig/%.pdf: fig/%.svg
	inkscape --without-gui -f $^ -D -A $@

data/%.eps: data/%.gp
	gnuplot $^

data/ycsb-overall/%.eps : data/ycsb-overall/%.gp
	gnuplot $^

data/ycsb-timeline/%.eps : data/ycsbd-timeline/%.gp
	gnuplot $^

data/ycsbc-lat/%.eps : data/ycsbc-lat/%.gp
	gnuplot $^

data/app/%.eps : data/app/%.gp
	gnuplot $^

data/datasets/%.eps : data/datasets/%.gp
	gnuplot $^

data/motiv/%.eps : data/motiv/%.gp
	gnuplot $^

draft: $(DEPS)
	echo -e '\\newcommand*{\\DRAFT}{}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

watermark: $(DEPS)
	echo -e '\\usepackage[firstpage]{draftwatermark}' >> rev.tex
	@TEXINPUTS="sty:" bin/latexrun $(BTEX) $(MAIN)

spell:
	@for i in *.tex fig/*.tex; do bin/aspell.sh $$i; done
	@for i in *.tex; do bin/double.pl $$i; done
	@for i in *.tex; do bin/abbrv.pl  $$i; done
	@bin/hyphens.sh *.tex

clean:
#	@bin/latexrun --clean
	latexmk -c
	rm -f abs.txt

distclean: clean
	rm -f code/*.tex

init:
	rm -f {code,fig,data}/ex-*
	perl -pi -e 's/^\\input{ex}/% \\input{ex}/g' $(MAIN).tex

abs.txt: abs.tex $(MAIN).tex
	#@bin/mkabstract $(MAIN).tex $< > $@

.PHONY: all help FORCE draft clean spell distclean init


==> ack.tex <==
dingyan: CUDA install
mingcong: valuable feedbacks 
